DFADD: The Diffusion and Flow-Matching Based Audio Deepfake Dataset

Mainstream zero-shot TTS production systems like Voicebox and Seed-TTS achieve human parity speech by leveraging Flow-matching and Diffusion models, respectively. Unfortunately, human-level audio synthesis leads to identity misuse and information security issues. Currently, many antispoofing models have been developed against deepfake audio. However, the efficacy of current state-of-the-art anti-spoofing models in countering audio synthesized by diffusion and flowmatching based TTS systems remains unknown. In this paper, we proposed the Diffusion and Flow-matching based Audio Deepfake (DFADD) dataset. The DFADD dataset collected the deepfake audio based on advanced diffusion and flowmatching TTS models. Additionally, we reveal that current anti-spoofing models lack sufficient robustness against highly human-like audio generated by diffusion and flow-matching TTS systems. The proposed DFADD dataset addresses this gap and provides a valuable resource for developing more resilient anti-spoofing models.

==> tables/unseen_results.tex <==
\definecolor{Gray}{gray}{0.85}
\newcolumntype{g}{>{\columncolor{Gray}}c}
\captionsetup[table]{skip=5pt}
\begin{table*}[t]
\centering
\fontsize{9}{10}\selectfont
\setlength\tabcolsep{5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
  \toprule
  \multicolumn{5}{c}{ASVspoof (All)} & \multicolumn{5}{c}{DFADD subets} \\
  \cmidrule(lr){2-3} \cmidrule(lr){4-14}
  & AASIST & AASIST-L & D1 & D2 & D3 & F1 & F2 & L-D1 & L-D2 & L-D3 & L-F1 & L-F2 \\
  \midrule
  VoiceBox & 42.59 & 47.62 & 53.77 & 64.70 & 50.13 & \textbf{36.69} & 60.80 & \textbf{43.97} & \textbf{38.94} & 63.31 & \cellcolor{Gray}\textbf{35.29} & 48.74   \\
  \midrule
  VoiceFlow & 50.41 & 41.33 & \textbf{34.70} & \textbf{33.06} & \textbf{33.06} & 42.96 & \textbf{24.80} & \textbf{25.61} & \cellcolor{Gray}\textbf{18.17} & \textbf{33.06} & \textbf{23.97} &  \textbf{23.15}  \\
  \midrule
  NaturalSpeech3 & 24.50 & 25.50 & 31.63 & 59.69 & 62.25 & \cellcolor{Gray}\textbf{18.38} & \textbf{24.50} & 31.62 & 30.62 & 43.87 & \textbf{21.93} & 34.18  \\
  \midrule
  CMTTS & 56.54 & 43.46 & \textbf{20.26} & \textbf{10.13} & \textbf{10.13} & \cellcolor{Gray}\textbf{0.00} & \cellcolor{Gray}\textbf{0.00} & \cellcolor{Gray}\textbf{0.00} & \cellcolor{Gray}\textbf{0.00} & \cellcolor{Gray}\textbf{0.00} & \textbf{5.89} & \cellcolor{Gray}\textbf{0.00} \\
  \midrule
  %DiffSpeech & 48.21 & 42.86 & 42.86 & 58.93 & \textbf{37.50} & 57.14 & 57.14 & \cellcolor{Gray}\textbf{35.71} & 74.42 & 57.14 & 64.28 & 57.14 \\
  %\midrule
  DiffProsody & 37.50 & 35.94 & 62.50 & \textbf{28.13} & \cellcolor{Gray}\textbf{25.00} & \cellcolor{Gray}\textbf{25.00} & \cellcolor{Gray}\textbf{25.00} & 50.00 & 50.00 & 62.50 & 62.50 & 50.00  \\
  \midrule
  DiffAR & 53.72 & 69.42 & 74.73 & \textbf{50.53} & {27.39} & \textbf{25.27} & \textbf{4.26} & \textbf{30.58} & 73.67 & \cellcolor{Gray}\textbf{3.19} & 81.11 & \textbf{50.53}  \\
  \midrule
  %ZETSpeech & 24.04 & 37.98 & 44.95 & 62.02 & 62.98 & 50.00 & \textbf{37.02} & 56.01 & 49.03 & \cellcolor{Gray}\textbf{31.01} & 62.98 & 43.99  \\
  %\midrule
  FlashSpeech & 63.87 & 54.20 & \cellcolor{Gray}\textbf{41.42} & 56.39 & 66.06 & 56.39 & 56.39 & 69.16 & 56.38 & 54.20 & \textbf{46.71} & 58.57 &  \\
  \bottomrule
\end{tabular}%
}
\caption{Performance comparison of spoofed speech detection (EER) between models trained on ASVspoof and DFADD datasets. Models surpassing those trained on ASVspoof are emphasized in bold. The top-performing models feature a gray background. Starting with L represents leave one out of the current subset result.}
\label{tab:unseen_results}
\end{table*}

% \captionsetup[table]{skip=5pt}
% \begin{table*}[t]
% \centering
% \fontsize{9}{10}\selectfont
% \setlength\tabcolsep{5pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccccccc}
%   \toprule
%   \multicolumn{5}{c}{ASVspoof (All)} & \multicolumn{5}{c}{DFADD} \\
%   \cmidrule(lr){2-3} \cmidrule(lr){4-14}
%   & AASIST & AASIST-L & D1 & D2 & D3 & F1 & F2 & F & G & H & E & H & All \\
%   \midrule
%   VoiceBox & 42.59 & 47.62 & 53.77 & 64.70 & 50.13 & 36.69 & 60.80 & - & - & - & - & - & 40.33 \\
%   \midrule
%   VoiceFlow & 50.41 & 41.33 & 34.70 & 33.06 & 33.06 & 42.96 & 24.80 & - & - & - & - & - & 26.43 \\
%   \midrule
%   NaturalSpeech3 & 24.50 & 25.50 & 31.63 & 59.69 & 62.25 & 18.38 & 24.50 & - & - & - & - & - & 31.63 \\
%   \midrule
%   CMTTS & 56.54 & 43.46 & 20.26 & 10.13 & 10.13 & 0.00 & 0.00 & - & - & - & - & - & 5.89 \\
%   \midrule
%   DiffSpeech & 48.21 & 42.86 & 42.86 & 58.93 & 37.50 & 57.14 & 57.14 & - & - & - & - & - & 57.14 \\
%   \midrule
%   DiffProsody & 37.50 & 35.94 & 62.50 & 28.13 & 25.00 & 25.00 & 25.00 & - & - & - & - & - & 62.50 \\
%   \midrule
%   DiffAR & 53.72 & 69.42 & 74.73 & 50.53 & 27.39 & 25.27 & 4.26 & - & - & - & - & - & 46.28 \\
%   \midrule
%   ZETSpeech & 24.04 & 37.98 & 44.95 & 62.02 & 62.98 & 50.00 & 37.02 & - & - & - & - & - & 42.03 \\
%   \midrule
%   FlashSpeech & 63.87 & 54.20 & 41.42 & 56.39 & 66.06 & 56.39 & 56.39 & - & - & - & - & - & 58.58 \\
%   \bottomrule
% \end{tabular}%
% }
% \caption{Comparison between codec models. "A$\sim$" signifies the AcademiCodec, "D$\sim$" represents the DAC, "E$\sim$" refers to the EnCodec. "None" means that no codec has been applied.}
% \label{tab: unseen_results}
% \end{table*}
